SMITE: Segment Me In TimE

Segmenting an object in a video presents significant challenges. Each pixel must be accurately labelled, and these labels must remain consistent across frames. The difficulty increases when the segmentation is with arbitrary granularity, meaning the number of segments can vary arbitrarily, and masks are defined based on only one or a few sample images. In this paper, we address this issue by employing a pre-trained text to image diffusion model supplemented with an additional tracking mechanism. We demonstrate that our approach can effectively manage various segmentation scenarios and outperforms state-of-the-art alternatives.

==> tables/ablation-old.tex <==
% \begin{table}[t!]
% \vspace{-20pt}
% \caption{\textbf{Segmentation results for non-textual semantic category.} 
% \name consistently outperforms SLiMe.\\}

% \label{table:Non-Textual Semantic Result}

% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{ccccccccccc}
% \toprule
%                       2D UNet & Inflated UNet & +Voting & +Regularization & Body & Light & Plate & Wheel & Window & Background & Average  \\ \midrule
% \cmark & \xmark & \xmark & \xmark & \textbf{62.7} & 80.4 & 67.0 & 57.2 & 81.4 & 97.3 & 74.3  \\
% \xmark & \cmark & \xmark & \xmark & \textbf{62.7} & 81.0 & \textbf{69.2} & 57.3 & 81.4 & 97.4 & 74.8  \\
% \xmark & \cmark & \cmark & \xmark & 58.3 & 78.1 & 52.6 & 50.8 & \textbf{82.0} & 97.3 & 69.9  \\
% \xmark & \cmark & \cmark & \cmark & 61.9 & \textbf{81.1} & 68.1 & \textbf{60.6} & 81.4 & \textbf{97.5} & \textbf{75.1}  \\
% \bottomrule
% \end{tabular}
% }

% \end{table}

\begin{table}[!t]
    % \caption{Global caption}
    \begin{minipage}{.49\linewidth}
      \caption{\textbf{Loss ablation.} When two losses are combined, the best performance is achieved.}
      \label{tab:loss-ab}
      \centering
      \footnotesize
      \setlength{\tabcolsep}{0.5em}
      \color{blue}
       \begin{tabular}{c|c}
\hline
 & \textbf{mIOU} \\ \hline
Baseline-I & 66.22 \\
+ inflated Unet & 69.36 \\
+ cross attention finetuning & _ \\
+ tracking & 72.64 \\
\hline
\rowcolor[HTML]{DAE8FC} 
+ regularization & \textbf{76.04}     \\ \hline
\end{tabular}
    \end{minipage}%
    \hspace{0.15cm}
    \begin{minipage}{.49\linewidth}
      \centering
        \caption{\textbf{Cross attention optimization} improves the quality of segmentation.}
        \label{tab:cross-ab}
        \footnotesize
        \setlength{\tabcolsep}{0.7em}
        \color{blue}
        \begin{tabular}{c|c}
\hline
\textbf{Finetuning Strategy}    & \textbf{mIOU} \\ \hline
Text Embedding                  & 74.86               \\ \hline
\rowcolor[HTML]{DAE8FC} 
\textbf{Cross Attention + Text} & \textbf{76.04}       \\ \hline
\end{tabular}
    \end{minipage} 
\end{table}

 



==> tables/baselines.tex <==
\begin{table}[t]
% \vspace{-20pt}
\centering
\footnotesize
\caption{\textbf{Quantitative Evaluation on \name-50 dataset.} 
The results are presented for each category (Faces, Horse, Cars, NonText) having 10 reference image during training.\\}
\label{tab:comparison}
\setlength{\tabcolsep}{0.23em}
\begin{tabular}{c|ccc|ccc|ccc|ccc}
\hline
                                   & \multicolumn{3}{c|}{\textbf{Faces}}                 & \multicolumn{3}{c|}{\textbf{Horses}}                & \multicolumn{3}{c|}{\textbf{Cars}}                  & \multicolumn{3}{c}{\textbf{Non-Text}}              \\ \cline{2-13} 
\multirow{-2}{*}{\textbf{Methods}} & $\textbf{F}_{meas.}$ & \textbf{mIOU}  & $\textbf{mVC}_{8}$ & $\textbf{F}_{meas.}$ & \textbf{mIOU}  & $\textbf{mVC}_{8}$ & $\textbf{F}_{meas.}$ & \textbf{mIOU}  & $\textbf{mVC}_{8}$ & $\textbf{F}_{meas.}$ & \textbf{mIOU} & $\textbf{mVC}_{8}$ \\ \hline
Baseline-I                              & 0.81               & 72.95          & zz            & 0.69               & 72.29          & zz            & 0.57               & 61.38          & zz            & 0.67                 & 66.69            & zz            \\
% Baseline-II                    & xx                 & xx             & zz            & xx                 & xx             & zz            & xx                 & xx             & zz            & xx                 & yy            & zz            \\
% XMem++                               & xx                 & xx             & zz            & xx                 & xx             & zz            & xx                 & xx             & zz            & xx                 & xx            & zz            \\
% VidSegDiff                        & xx                 & xx             & zz            & xx                 & xx             & zz            & xx                 & xx             & zz            & xx                 & yy            & zz            \\
GSAM2                       & 0.73               & 63.28          & zz            & \textbf{0.81}               & \textbf{78.31}          & zz            & 0.64               & 63.56          & zz            & -                 & -            & -            \\ \hline
\rowcolor[HTML]{DAE8FC} 
\textbf{Ours}                      & \textbf{0.89}      & \textbf{77.28} & zz            & 0.77      & 76.72 & zz            & \textbf{0.82}      & \textbf{75.10} & zz            & 0.77                 & 73.08            & zz            \\ \hline
\end{tabular}
\end{table}







% \begin{table}[t!]
% \vspace{-20pt}
% \caption{\textbf{Performance comparison of models.} 
% The results are presented for each category (Faces, Horse, Cars) and evaluated using F-Measure and MIoU metrics. The table shows baseline models, including SLiMe, CoTracker, and Grounded SAM2. \name demonstrates superior performance across all categories.\\}

% \label{table:performance_comparison}

% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lcccccc}
% \toprule
%                       & \multicolumn{2}{c}{Faces} & \multicolumn{2}{c}{Horse} & \multicolumn{2}{c}{Cars} \\ 
%                       & F\_Measure & MIoU & F\_Measure & MIoU & F\_Measure & MIoU \\ \midrule
% VidSeg\_diffusion     & - & - & - & - & - & - \\
% SLIME                 & 0.81 & 72.95 & 0.73 & 74.07 & 0.60 & 66.38 \\
% SLIME+CoTracker       & - & - & - & - & - & - \\
% Grounded SAM2         & 0.73 & 63.28 & 0.72 & 68.08 & 0.60 & 59.18 \\
% \hline
% \rowcolor[HTML]{DAE8FC}
% Ours                  & \textbf{0.89} & \textbf{77.28} & \textbf{0.73} & \textbf{75.49} & \textbf{0.70} & \textbf{71.97} \\ 
% \bottomrule
% \end{tabular}
% }

% \end{table}


==> tables/celeba_hq.tex <==
\begin{table}[t!]
\caption{\textbf{Segmentation results on CelebAMask-HQ10.} The first two rows represent the 1-sample setting, and the remaining rows represent the 10-sample setting. $^\star$ denotes supervised methods. Our approach achieves competitive results and demonstrates strong overall performance.}
\label{table:celebe_result}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cccccccccc|c}
\hline
                      & Cloth & Eyebrow & Ear  & Eye  & Hair & Mouth & Neck & Nose & Face & Background & Average \\ \hline
$\text{SegGPT}^\star$  & 24.0  & 48.8    & 32.3 & 51.7 & 82.7 & 66.7  & 77.3 & 73.6 & 85.7 & 28.0       & 57.1    \\
OIParts                & 60.9  & 48.1    & 63.4 & 65.0 & 82.2 & 79.1  & 76.9 & 74.0 & 86.5 & 83.8       & 72.0    \\ \hline
ReGAN                  & 15.5  & \textbf{68.2} & 37.3 & \textbf{75.4} & 84.0 & \textbf{86.5} & \textbf{80.3} & \textbf{84.6} & 90.0 & 84.7       & 69.9    \\
SegDDPM                & 61.6  & 67.5    & \textbf{71.3} & 73.5 & \textbf{86.1} & 83.5  & 79.2 & 81.9 & 89.2 & 86.5       & \textbf{78.0}    \\
SLiMe                  & 63.1 $\pm$ 1.6 & 62.0 $\pm$ 1.6 & 64.2 $\pm$ 1.9 & 65.5 $\pm$ 3.0 & 85.3 $\pm$ 0.4 & 82.1 $\pm$ 1.6 & 79.4 $\pm$ 2.2 & 79.1 $\pm$ 1.4 & 88.8 $\pm$ 0.2 & \textbf{87.1 $\pm$ 0.0} & 75.7 $\pm$ 0.4 \\ 
\rowcolor[HTML]{DAE8FC} 
Ours                   & \textbf{63.4} & 67.8 & 66.1 & 70.9 & 84.6 & 84.7 & \textbf{80.3} & 83.2 & \textbf{90.8} & 86.2 & 77.8 \\ \hline
\end{tabular}
}
\end{table}



% \begin{table}[t!]
% \caption{\textbf{Segmentation results on CelebAMask-HQ10.} The first two rows represent the 1-sample setting, and the remaining rows represent the 10-sample setting. $^\star$ denotes supervised methods. Our approach achieves competitive results and demonstrates strong overall performance.}
% \label{table:celebe_result}
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{cccccccccccc}
% \toprule
%                       & Cloth & Eyebrow & Ear  & Eye  & Hair & Mouth & Neck & Nose & Face & Background & Average \\ 
% \midrule
% $\text{SegGPT}^\star$ & 24.0 & 48.8 & 32.3 & 51.7 & 82.7 & 66.7 & 77.3 & 73.6 & 85.7 & 28.0 & 57.1 \\
% OIParts        & 60.9 & 48.1 & 63.4 & 65.0 & 82.2 & 79.1 & 76.9 & 74.0 & 86.5 & 83.8 & 72.0 \\ 
% \midrule
% ReGAN                 & 15.5 & \textbf{68.2} & 37.3 & \textbf{75.4} & 84.0 & \textbf{86.5} & \textbf{80.3} & \textbf{84.6} & 90.0 & 84.7 & 69.9 \\
% SegDDPM               & 61.6 & 67.5 & \textbf{71.3} & 73.5 & \textbf{86.1} & 83.5 & 79.2 & 81.9 & 89.2 & 86.5 & \textbf{78.0} \\
% SLiMe        & 63.1 $\pm$ 1.6 & 62.0 $\pm$ 1.6 & 64.2 $\pm$ 1.9 & 65.5 $\pm$ 3.0 & 85.3 $\pm$ 0.4 & 82.1 $\pm$ 1.6 & 79.4 $\pm$ 2.2 & 79.1 $\pm$ 1.4 & 88.8 $\pm$ 0.2 & \textbf{87.1 $\pm$ 0.0} & 75.7 $\pm$ 0.4 \\ 
% Ours       & \textbf{63.4 $\pm$ 2.3} & 67.8 $\pm$ 1.6 & 66.1 $\pm$ 0.4 & 70.9 $\pm$ 0.6 & 84.6 $\pm$ 0.3 & 84.7 $\pm$ 0.8 & \textbf{80.3 $\pm$ 0.5} & 83.2 $\pm$ 0.4 & \textbf{90.8 $\pm$ 0.3} & 86.2 $\pm$ 0.2 & 77.8 $\pm$ 0.1 \\ 
% \bottomrule
% \end{tabular}
% }
% \end{table}


